Creating a Relational Distributed Object Store

In and of itself, data storage has apparent business utility. But when we can convert data to information, the utility of stored data increases dramatically. It is the layering of relation atop the data mass that is the engine for such conversion. Frank relation amongst discrete objects sporadically ingested is rare, making the process of synthesizing such relation all the more challenging, but the challenge must be met if we are ever to see an equivalent business value for unstructured data as we already have with structured data. This paper describes a novel construct, referred to as a relational distributed object store (RDOS), that seeks to solve the twin problems of how to persistently and reliably store petabytes of unstructured data while simultaneously creating and persisting relations amongst billions of objects.

==> Makefile <==
MAKE=make
PDFLATEX=pdflatex
RTFLATEX=latex2rtf
BIBTEX=bibtex

PAPER=doc
BIBFILE=master.bib

TEXFILES = $(wildcard *.tex)

all: subdirs $(PAPER).pdf

$(PAPER).pdf: $(TEXFILES) $(BIBFILE)
	$(PDFLATEX) $(PAPER)
	$(BIBTEX) $(PAPER)
	$(PDFLATEX) $(PAPER)
	$(PDFLATEX) $(PAPER)
#	$(RTFLATEX) $(PAPER)

subdirs:
	$(MAKE) -C fig

clean:
	$(MAKE) -C fig clean 
	/bin/rm -rf auto *.aux *~ *.log *.lot *.lof *.toc *.blg *.bbl *.out

clean-all:\
	clean
	/bin/rm -f $(PAPER).pdf $(PAPER).rtf

